Bayesian Hierarchical Modelling of Noisy Gamma Processes: Model Formulation, Identifiability, Model Fitting, and Extensions to Unit-to-Unit Variability

The gamma process is a natural model for monotonic degradation processes. In practice, it is desirable to extend the single gamma process to incorporate measurement error and to construct models for the degradation of several nominally identical units. In this paper, we show how these extensions are easily facilitated through the Bayesian hierarchical modelling framework. Following the precepts of the Bayesian statistical workflow, we show the principled construction of a noisy gamma process model. We also reparameterise the gamma process to simplify the specification of priors and make it obvious how the single gamma process model can be extended to include unit-to-unit variability or covariates. We first fit the noisy gamma process model to a single simulated degradation trace. In doing so, we find an identifiability problem between the volatility of the gamma process and the measurement error when there are only a few noisy degradation observations. However, this lack of identifiability can be resolved by including extra information in the analysis through a stronger prior or extra data that informs one of the non-identifiable parameters, or by borrowing information from multiple units. We then explore extensions of the model to account for unit-to-unit variability and demonstrate them using a crack-propagation data set with added measurement error. Lastly, we perform model selection in a fully Bayesian framework by using cross-validation to approximate the expected log probability density of new observation. We also show how failure time distributions with uncertainty intervals can be calculated for new units or units that are currently under test but are yet to fail.

==> stan_fit_pp_both_table.tex <==
\begin{table}
\centering
\caption{\label{tab:pp_both}Partial output from fitting a BHM to the noisy data of Fig.~\ref{fig:RP_w_noise} where both the coefficient of variation $\nu_j$ and the mean wear rate $\mu_j$ varies between units. Only statistics for Units~1--4 are shown.}
\centering
\begin{tabular}[t]{lrrrrrr}
\toprule
Parameter & Mean & 2.5\% & 50\% & 97.5\% & $n_{\small{\mbox{eff}}}$ & $\hat{R}$\\
\midrule
\cellcolor{gray!10}{$\sigma$} & \cellcolor{gray!10}{0.03} & \cellcolor{gray!10}{0.02} & \cellcolor{gray!10}{0.03} & \cellcolor{gray!10}{0.04} & \cellcolor{gray!10}{1656} & \cellcolor{gray!10}{1.01}\\
$\nu_1$ & 0.18 & 0.06 & 0.19 & 0.31 & 1069 & 1.01\\
\cellcolor{gray!10}{$\nu_2$} & \cellcolor{gray!10}{0.19} & \cellcolor{gray!10}{0.08} & \cellcolor{gray!10}{0.19} & \cellcolor{gray!10}{0.32} & \cellcolor{gray!10}{1353} & \cellcolor{gray!10}{1.01}\\
$\nu_3$ & 0.20 & 0.07 & 0.20 & 0.33 & 1158 & 1.01\\
\cellcolor{gray!10}{$\nu_4$} & \cellcolor{gray!10}{0.20} & \cellcolor{gray!10}{0.07} & \cellcolor{gray!10}{0.20} & \cellcolor{gray!10}{0.33} & \cellcolor{gray!10}{1092} & \cellcolor{gray!10}{1.01}\\
\addlinespace
$\mu_1$ & 0.37 & 0.26 & 0.37 & 0.49 & 2966 & 1.00\\
\cellcolor{gray!10}{$\mu_2$} & \cellcolor{gray!10}{0.44} & \cellcolor{gray!10}{0.33} & \cellcolor{gray!10}{0.43} & \cellcolor{gray!10}{0.60} & \cellcolor{gray!10}{3426} & \cellcolor{gray!10}{1.00}\\
$\mu_3$ & 0.36 & 0.25 & 0.36 & 0.49 & 1795 & 1.00\\
\cellcolor{gray!10}{$\mu_4$} & \cellcolor{gray!10}{0.35} & \cellcolor{gray!10}{0.23} & \cellcolor{gray!10}{0.35} & \cellcolor{gray!10}{0.48} & \cellcolor{gray!10}{1242} & \cellcolor{gray!10}{1.01}\\
$\mu_\mu$ & 0.40 & 0.33 & 0.40 & 0.51 & 6667 & 1.00\\
\addlinespace
\cellcolor{gray!10}{$\sigma_\mu$} & \cellcolor{gray!10}{0.07} & \cellcolor{gray!10}{0.01} & \cellcolor{gray!10}{0.07} & \cellcolor{gray!10}{0.19} & \cellcolor{gray!10}{451} & \cellcolor{gray!10}{1.01}\\
$\mu_\nu$ & 0.19 & 0.09 & 0.19 & 0.29 & 810 & 1.01\\
\cellcolor{gray!10}{$\sigma_\nu$} & \cellcolor{gray!10}{0.04} & \cellcolor{gray!10}{0.00} & \cellcolor{gray!10}{0.03} & \cellcolor{gray!10}{0.11} & \cellcolor{gray!10}{808} & \cellcolor{gray!10}{1.01}\\
\bottomrule
\end{tabular}
\end{table}

